Controlled Text Generation for Black-box Language Models via Score-based Progressive Editor

Controlled text generation is very important for the practical use of language models because it ensures that the produced text includes only the desired attributes from a specific domain or dataset. Existing methods, however, are inapplicable to black-box models or suffer a significant trade-off between controlling the generated text and maintaining its fluency. This paper introduces the Score-based Progressive Editor (ScoPE), a novel approach designed to overcome these issues. ScoPE modifies the context at the token level during the generation process of a backbone language model. This modification guides the subsequent text to naturally include the target attributes. To facilitate this process, ScoPE employs a training objective that maximizes a target score, thoroughly considering both the ability to guide the text and its fluency. Experimental results on diverse controlled generation tasks demonstrate that ScoPE can effectively regulate the attributes of the generated text while fully utilizing the capability of the backbone large language models. Our codes are available at \url{https://github.com/ysw1021/ScoPE}.

==> sections/A1.Tech_for_stable_training.tex <==
\section{Techniques for Stable Training of ScoPE} \label{stable_training}
% Techniques for stable training are described in the Appendix. 

% \paragraph{Techniques for stable training}
In this work, we employ four techniques for training stability: 
1) teacher-forcing training framework, 
2) parameter initialization with MLM fine-tuned for the target corpus, 
3) providing training signals only at the positions of edited tokens, 
4) clipping the score disparity between input and edited texts.

==> tables/category_llama2_camera.tex <==
\begin{table*}[t]
\centering
{\footnotesize\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l||cccc|cccc}
\toprule
 \multirow{2}{*}{\textbf{Methods}} & \multicolumn{4}{c|}{$\textbf{PPL}$ $\downarrow$} & \multicolumn{4}{c}{\textbf{MAUVE} $\uparrow$}          \\
             &  \textbf{Camera} & \textbf{Videogame} & \textbf{Grocery} & \textbf{Music} & \textbf{Camera} &\textbf{Videogame} & \textbf{Grocery} & \textbf{Music}   \\ \hline
LLaMA2-7B  &  11.90& \textbf{12.34}& \textbf{10.51}& \textbf{12.06}
& 0.6643& 0.1434&  0.0654& 0.0290\\
ScoPE ($N$=1) &  13.06&  14.73& 14.22& 16.51
& 0.7159& 0.5658&  0.4099& 0.3030\\
ScoPE ($N$=5) &  11.47&  12.67& 12.38& 14.04
& 0.7415& 0.6621&  \textbf{0.5439}& 0.4740
\\
ScoPE ($N$=10) &  \textbf{11.46}&  12.52& 12.12& 13.96& \textbf{0.7600}& \textbf{0.6654}&  0.5221& \textbf{0.4758}\\ 
\bottomrule
\end{tabular}
}}
\caption{Experimental results for category controlled generation targeting the Camera attributes. LLaMA2-7B is utilized for both trainset construction and backbone model at the generation process. $N$ denotes the number of iterative edits performed on the input text.}
\label{table1}
\end{table*}

==> tables/sentiment_comparison_neg.tex <==
\begin{table}[t]
\centering
{\footnotesize\resizebox{\columnwidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l||cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c|}{$\textbf{PPL}$ $\downarrow$} & \multicolumn{2}{c|}{\textbf{Acc. 1} $\uparrow$} & \multicolumn{2}{c}{\textbf{Acc. 2} $\uparrow$} \\
& \textbf{Pos.} & \textbf{Neg.} & \textbf{Pos.} & \textbf{Neg.} & \textbf{Pos.} & \textbf{Neg.} \\ \hline
DExperts & 44.83& 69.03& 91.38& 99.37& 90.52& 97.87\\
GeDi & 80.51& 94.64& 73.82& 95.58& 74.91& 91.49\\
Mix\&Match & 16.4& 16.55& 55.82& 92.57& 20.14& 66.65\\ \hline
ScoPE ($N$=10)& 12.6& 12.91
& 54.41& 88.01& 55.9& 87.88
\\
 $+$ EDG & 12.79& 13.08& 79.59& 95.4& 81.84& 94.43\\
\bottomrule
\end{tabular}
}}
\caption{Experimental results for sentiment controlled text generation targeting the negative attribute comparing with prior works. GPT2-XL is utilized for both ScoPE trainset construction and the backbone model for the ScoPE generation process. The accuracy from the discriminator used to ScoPE training is denoted as \textbf{Acc. 1}, while the accuracy from the discriminator not used to ScoPE training is denoted as \textbf{Acc. 2}. EDG refers to external discriminator guidance.}
\label{table_sentiment_comparision_neg}
\end{table}
